KubeFence: Security Hardening of the Kubernetes Attack Surface

Kubernetes (K8s) is widely used to orchestrate containerized applications, including critical services in domains such as finance, healthcare, and government. However, its extensive and feature-rich API interface exposes a broad attack surface, making K8s vulnerable to exploits of software vulnerabilities and misconfigurations. Even if K8s adopts role-based access control (RBAC) to manage access to K8s APIs, this approach lacks the granularity needed to protect specification attributes within API requests. This paper proposes a novel solution, KubeFence, which implements finer-grain API filtering tailored to specific client workloads. KubeFence analyzes Kubernetes Operators from trusted repositories and leverages their configuration files to restrict unnecessary features of the K8s API, to mitigate misconfigurations and vulnerabilities exploitable through the K8s API. The experimental results show that KubeFence can significantly reduce the attack surface and prevent attacks compared to RBAC.

==> yaml_files/generated_values.tex <==
\begin{lstlisting}[language=yaml, caption={Set of Generated Values Files}, label={lst:generated_values}]

DEFAULT VALUES FILE
backendStore:
  databaseMigration: false
  databaseConnectionCheck: false
  postgres:
    enabled: false

PARAMETRIZED VALUES FILE
backendStore:
  databaseMigration: false,true
  databaseConnectionCheck: false,true
  postgres:
    enabled: false,true

SET OF GENERATED VALUES FILES
backendStore:
  databaseMigration: false
  databaseConnectionCheck: false
  postgres:
    enabled: false
--------------------    
backendStore:
  databaseMigration: true
  databaseConnectionCheck: true
  postgres:
    enabled: true
\end{lstlisting}
